Pure Differential Privacy from Secure Intermediaries

Recent work in differential privacy has explored the prospect of combining local randomization with a secure intermediary. Specifically, there are a variety of protocols in the secure shuffle model (where an intermediary randomly permutes messages) as well as the secure aggregation model (where an intermediary adds messages). Most of these protocols are limited to approximate differential privacy. An exception is the shuffle protocol by Ghazi, Golowich, Kumar, Manurangsi, Pagh, and Velingker (arXiv:2002.01919): it computes bounded sums under pure differential privacy. Its additive error is $\tilde{O}(1/\varepsilon^{3/2})$, where $\varepsilon$ is the privacy parameter. In this work, we give a new protocol that ensures $O(1/\varepsilon)$ error under pure differential privacy. We also show how to use it to test uniformity of distributions over $[d]$. The tester's sample complexity has an optimal dependence on $d$. Our work relies on a novel class of secure intermediaries which are of independent interest.

==> simulate-shuffle.tex <==
\section{Simulating Secure Shuffling via Secure Aggregation}

In this section, we show how to shuffle $n$ values in the secure aggregation model. We first recap a naive approach that scales poorly with the message length and then provide an alternative approach for long messages.

\biganote{formalize}

idea: for each potential message value $v\in[d]$, count the occurrences of $v$.

costly because we need to perform $d$ counts which could be expensive either in terms of round complexity or in terms of required parallel computations

\biganote{formalize}

idea: first compute $s\gets $ the sum of $n$ values. then each user picks a random number in $[\ell]$. in round $t$, if the user's chosen number matches $t$ then they input their value to the sum primitive. otherwise they input the negation. If the number of rounds $\ell$ is sufficiently large, users pick unique rounds to report their true value. So the view of the analyzer is $s$ followed by a list of sums where most are just $-s$ and the others have the form $-s+2x$ where $x$ is a user's value. They can recover the multiset of user values through addition and division by 2.
